Simultaneous X-ray and optical variability of M dwarfs observed with eROSITA and TESS

We study variability through simultaneous optical and X-ray observations for the first time in a statistical sample of 256 M dwarfs. Such observations are required to constrain the flare frequency and energetics and to understand the physics of flares. Using light curves from extended ROentgen Survey with an Imaging Telescope Array (eROSITA) on board the Russian Spektrum-Roentgen-Gamma mission (SRG) and the Transiting Exoplanet Survey Satellite (TESS), we identify 256 M dwarfs with simultaneous detections. The 25 brightest or most variable in X-rays are selected. Stellar parameters are obtained from Gaia and 2MASS, while X-ray fluxes are derived from eROSITA count rates. Proximity (<100 pc), fast rotation (P_rot < 9 d), and high flare frequency characterize our sample. Optical and X-ray duty cycles correlate positively, with faster rotators exhibiting more variability. Stars with frequent X-ray flares often coincide with optical flares. Analyzing individual X-ray flares is hindered by eROSITA's low cadence, mitigated by leveraging TESS optical flares and solar flare knowledge. An exponential fit to 21 X-ray light curves post-optical flares reveals a correlation between X-ray and optical flare energies. Despite uncertainties due to poor eROSITA sampling, our study underscores the significance of simultaneous all-sky surveys in diverse wavelengths for unprecedented insights into stellar variability.

==> exp_fits.tex <==
\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC140758953_em03_2328.7460711956955-2332.5787086052114.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC150359500_em02_2144.5162382538715-2149.2052227654494.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC167812509_em03_2350.9203598271124-2355.587026493624.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC167894019_em02_2166.204164636787-2169.9439209942484.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC220473309_em02_2066.702884722501-2074.744551389478.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC220473309_em03_2241.6096876696683-2246.9430210026912.pdf}}
  }
  \caption{\textcolor{teal}{14 of the best fitting exponential curves from our sample.}}
  \label{}
\end{figure*}

\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC277298771_em02_2146.7098534922116-2158.0431868257.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC277298771_em03_2333.8564375291407-2339.0818238044158.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC278731274_em03_2327.088636886794-2331.421970219817.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC278825715_em03_2329.088636886794-2332.578487205468.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC31381302_em02_2127.252547695767-2137.5442143622786.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC31381302_em03_2301.7477979892865-2305.9884087063097.pdf}}
  }
  \caption{\textcolor{teal}{14 of the best fitting exponential curves from our sample.}}
  \label{}
\end{figure*}

\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC55497266_em02_2037.370440817438-2046.370440817438.pdf
}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits/TIC55497266_em03_2221.7753945193253-2227.571813164617.pdf
}}
  }
  \caption{\textcolor{teal}{14 of the best fitting exponential curves from our sample.}}
  \label{}
\end{figure*}



==> exp_fits_new.tex <==
\begin{figure*}[h]
\centering
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC140758953_em03_2328.936_2.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC140758953_em03_2331.548_1.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC150359500_em02_2145.755_2.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC150359500_em02_2147.257_1.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC167812509_em03_2353.698_1.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC167894019_em02_2166.905_1.pdf}}
}
\caption{\textcolor{teal}{eRASS light curves illustrating our estimate of the X-ray flare peak (red data point) as explained in Sect.~\ref{subsubsect:xrayflare_peakestimate} and the exponential fit to the flare decay (black curve) described in Sect.~\ref{subsubsect:xrayflare_expfit}.}}
%\textcolor{orange}{\bf BS-comment: Caption text missing. In all subsequent figures D1, put the caption "continued".}}
\label{fig:exp-fits}
\end{figure*}

\begin{figure*}[h]
\centering
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC167894019_em02_2167.776_2.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC220473309_em02_2070.715_1.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC220473309_em02_2071.572_2.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC220473309_em03_2245.54_2.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC220473309_em03_2246.004_1.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em02_2146.843_3.pdf}}
}
\addtocounter{figure}{-1}
\caption{Continued}
\label{fig:exp-fits-2}
\end{figure*}

\begin{figure*}[h]
\centering
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em02_2147.488_1.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em02_2149.122_2.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em02_2150.009_5.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em02_2150.731_6.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em02_2155.959_4.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em03_2334.251_1.pdf}}
}
\addtocounter{figure}{-1}
\caption{Continued}
\label{fig:exp-fits-3}
\end{figure*}

\begin{figure*}[h]
\centering
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em03_2334.595_2.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC277298771_em03_2338.056_3.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC278725797_em03_2328.794_1.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC278731274_em03_2329.204_1.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC278825715_em03_2329.769_2.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC278825715_em03_2330.31_1.pdf}}
}
\addtocounter{figure}{-1}
\caption{Continued}
\label{fig:exp-fits-4}
\end{figure*}

\begin{figure*}[h]
\centering
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC31381302_em02_2132.836_1.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC31381302_em03_2301.984_1.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC33866201_em02_2149.016_1.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC55497266_em02_2037.512_3.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC55497266_em02_2041.92_2.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC55497266_em02_2042.174_1.pdf}}
}
\addtocounter{figure}{-1}
\caption{Continued}
\label{fig:exp-fits-5}
\end{figure*}

\begin{figure*}[h]
\centering
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC55497266_em02_2045.845_4.pdf}}
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC55497266_em03_2225.239_1.pdf}}
}
\parbox{\textwidth}{
	\parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_new/TIC55497266_em03_2226.882_2.pdf}}
 }
\addtocounter{figure}{-1}
\caption{Continued}
\label{fig:exp-fits-6}
\end{figure*}


==> exp_fits_okay.tex <==
\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_okay/tic140758953e3_1.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_okay/tic277298771e2_1.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/exp_fits_okay/tic55497266e3_1.pdf}}
  }
  \caption{\textcolor{teal}{3 exponential fits found to be suitable by eye.}}
  \label{fig:exp-fits-okay}
\end{figure*}

==> flat_lc_tess.tex <==
\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC140758953_em03_2328.7460711956955-2332.5787086052114.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC141156752_em03_2316.2462510028854-2323.079584336374.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC150359500_em02_2144.5162382538715-2149.2052227654494.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC167812509_em03_2350.9203598271124-2355.587026493624.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC167894019_em02_2166.204164636787-2169.9439209942484.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC220473309_em02_2066.702884722501-2074.744551389478.pdf}}
  }
  \caption{\textcolor{teal}{Flattened TESS light curves with flares and eRASS light curves. The eRASS points significantly above the quiescent level (purple), also named as the ``X-ray flare points", are marked in red. The TESS flare points are marked in dark blue. X-ray flare points around which TESS flares were found are marked as green squares, and the vertical bins of width 1eROday in which they lie are marked with dashed blue lines} \textcolor{blue}{I've added only the light curves with TESS flares, do you think it's best to add all of them? (there are 51, and I'm not sure I can upload more than 40 to a folder}}
  \label{fig:all-lc}
\end{figure*}

\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC220473309_em03_2241.6096876696683-2246.9430210026912}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC277298771_em02_2146.7098534922116-2158.0431868257.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC277298771_em03_2324.4151571379043-2332.5786511876304.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC277298771_em03_2333.8564375291407-2339.0818238044158.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC278725797_em03_2326.588636886794-2330.921970219817.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC278731274_em02_2145.5363411856815-2148.8696745187044.pdf}}
  }
  \addtocounter{figure}{-1}
  \caption{Continued}
  \label{fig:flat-lc-2}
\end{figure*}

\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC278731274_em03_2327.088636886794-2331.421970219817.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC278825715_em03_2329.088636886794-2332.578487205468.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC31381302_em02_2127.252547695767-2137.5442143622786.pdf }}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC31381302_em03_2301.7477979892865-2305.9884087063097.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC33866201_em02_2148.880515933037-2152.2138492665254.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC350145729_em02_2194-2198.932654767297.pdf}}
  }
  \addtocounter{figure}{-1}
  \caption{Continued}
  \label{fig:flat-lc-3}
\end{figure*}

\begin{figure*}[h]
  \centering
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC350145729_em03_2361.773529556616-2382.0883719748817.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC55497266_em02_2037.370440817438-2046.370440817438.pdf}}
  }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/flat_lc/TIC55497266_em03_2221.7753945193253-2227.571813164617.pdf}}
  }
  \addtocounter{figure}{-1}
  \caption{Continued}
  \label{fig:flat-lc-4}
\end{figure*}



==> interesting_flares.tex <==
\begin{figure*}%[h]
  \centering
  % \parbox{\textwidth}{
  %   \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/interesting_flares/tic150359500e2_1.pdf}}
  %   \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/interesting_flares/tic150359500e2_2.pdf}}
  % }
  % \parbox{\textwidth}{
  %   \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/interesting_flares/tic150359500e2_3.pdf}}
  %   \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/interesting_flares/tic278731274e3_1.pdf}}
  % }
  % \parbox{\textwidth}{
  %   \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/interesting_flares/tic278731274e3_2.pdf}}
  % }
  \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/interesting_flares/TIC150359500_em02_full_fit.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/interesting_flares/TIC278731274_em03_full_fit:.pdf}}
  }

  \caption{\textcolor{teal}{5 complex flares\textcolor{red}{Carry out an exponential fit for the event on TIC2787 including ALL red bins from the beginning (and maybe some bins afterwards). Calculate its energy.\textcolor{teal}{E from curve normalized to R0 and Rqui respectively: 2.991e+35 and 2.865e+35 erg} For the flare on TIC 105 integrate under the observed LC over all red bins and calculate the energy.\textcolor{teal}{E from linearly interpolated curve normalized to R0 and Rqui respectively:4.563e+34 and  4.753e+34 erg}\textcolor{blue}{The plots are just to show what the curves under which I integrate look like, they will of coursse be modified if they go into the paper}}}}
  \label{fig:interesting-flares}
\end{figure*}

\begin{figure*}[h]
  \centering
    % \parbox{\textwidth}{
    % \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/tic150359500e2_paper_plot_flat.pdf}}
    % \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/tic278731274e3_paper_plot_flat.pdf}}
        \parbox{\textwidth}{
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/tic150359500e2_paper_plot.pdf}}
    \parbox{0.5\textwidth}{\includegraphics[width=0.5\textwidth]{images/tic278731274e3_paper_plot.pdf}}
  }
  \end{figure*}

==> tables/erass-tess-dates.tex <==
\begin{table*}[ht!]\label{erass-tess-dates}
  \begin{center}
    \caption{Observation start and stop dates of eRASS 2, eRASS 3 and TESS sectors 27-39}
    \label{tab:erass-tess-dates}
    \begin{tabular}{c|c|c|c|c|c} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
      \textbf{Survey} & \textbf{Start date} & \textbf{Stop date}& \textbf{Survey} & \textbf{Start date} & \textbf{Stop date}\\
      \hline
      eRASS 2 & 11.06.2020 & 15.12.2020 & TESS s27-39 & 04.07.2020 & 24.06.2021\\
      eRASS 3 & 15.12.2020 & 16.06.2021 & & & \\
    \end{tabular}
  \end{center}
\end{table*}

==> tables/star_properties.tex <==
\begin{table}[!ht]
    \centering
    \begin{adjustbox}{angle=90}
    \small
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
        TIC ID & P_{rot,eRASS2} & \nu_{TESS,DC,eRASS2} & \nu_{TESS,DC,eRASS3} & \nu_{TESS,DC,mean} & \nu_{TESS,eRASS2} & \nu_{TESS,eRASS3} & \nu_{TESS,mean} & \nu_{x,eRASS2} & \nu_{x,eRASS3} & \nu{x,mean} & R_{qui,eRASS2} & R_{qui,eRASS3} & R_{qui,mean} & P_{Rot,eRASS3} & P_{Rot,mean} \\ \hline
        TIC140758953 & 1.3744605 & 0.009327758 & 0.018104367 & 0.0137160625 & 0.92338735 & 1.0216253 & 0.9725063 & 0.22222222 & 0.2777778 & 0.25 & 0.0044154855 & 0.027406696 & 0.015911091 & 1.3666141 & 1.3705373 \\ \hline
        TIC141156752 & 1.4165025 & 0.024760833 & 0.019371346 & 0.022066088 & 0.80945545 & 0.73184633 & 0.77065086 & 0.33333334 & 0.35714287 & 0.3452381 & 0.025535543 & 0.0262952 & 0.025915371 & 1.888818 & 1.6526603 \\ \hline
        TIC141422340 & 13.640042 & 0.0062981104 & 0.0022975302 & 0.0042978204 & 0.50018185 & 0.2063596 & 0.35327074 & 0.12 & 0.05882353 & 0.089411765 & 0.016284266 & 0.005677114 & 0.01098069 & 11.3962145 & 12.518128 \\ \hline
        TIC142052608 & 2.9840138 & 0.0027054448 & 0.0 & 0.0013527224 & 0.24291939 & 0.0 & 0.12145969 & 0.051282052 & 0.21212122 & 0.13170163 & 0.0040322538 & 0.011087426 & 0.00755984 & 2.936474 & 2.960244 \\ \hline
        TIC150301109 & 2.6214688 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.071428575 & 0.14285715 & 0.10714286 & 0.028582865 & 0.028569115 & 0.02857599 & 1.0073314 & 1.8144001 \\ \hline
        TIC150359500 & 1.0294805 & 0.12810536 & ~ & 0.12810536 & 4.9491262 & ~ & 4.9491262 & 0.5 & 0.4318182 & 0.4659091 & 2.5173736 & 1.8275822 & 2.172478 & ~ & 1.0294805 \\ \hline
        TIC167812509 & 0.3359067 & 0.0068863747 & 0.0041753654 & 0.00553087 & 0.7086525 & 0.42870507 & 0.5686788 & 0.21875 & 0.31034482 & 0.2645474 & 0.01840663 & 0.0050214347 & 0.011714032 & 0.33638772 & 0.33614722 \\ \hline
        TIC167894019 & 3.9120774 & 0.018982535 & 0.025060913 & 0.022021724 & 0.8203455 & 1.750634 & 1.2854897 & 0.1724138 & 0.48 & 0.3262069 & 0.02424524 & 0.06220448 & 0.04322486 & 1.1882089 & 2.5501432 \\ \hline
        TIC177257889 & 11.651164 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.06382979 & 0.056603774 & 0.06021678 & 0.0056922324 & 0.017261982 & 0.011477107 & 10.20642 & 10.928792 \\ \hline
        TIC220395392 & ~ & ~ & 0.0041771093 & 0.0041771093 & ~ & 0.40011987 & 0.40011987 & 0.41304347 & 0.29032257 & 0.35168302 & 0.3254613 & 0.3054184 & 0.31543985 & 5.0658875 & 5.0658875 \\ \hline
        TIC220473309 & 8.795243 & 0.10683054 & 0.17072399 & 0.13877727 & 3.7375443 & 7.2866673 & 5.512106 & 0.6744186 & 0.4375 & 0.5559593 & 3.6051366 & 4.6029596 & 4.1040483 & 8.601143 & 8.698194 \\ \hline
        TIC260189734 & 17.288353 & 0.0029218409 & 0.0060728746 & 0.0044973576 & 0.26095992 & 0.18186726 & 0.22141358 & 0.33333334 & 0.44117647 & 0.3872549 & 0.023634668 & 0.06180969 & 0.04272218 & 15.586027 & 16.43719 \\ \hline
        TIC260352702 & ~ & ~ & 0.006136852 & 0.006136852 & ~ & 0.8837255 & 0.8837255 & 0.045454547 & 0.03448276 & 0.03996865 & 0.04211879 & 0.0145110125 & 0.028314902 & 1.0033232 & 1.0033232 \\ \hline
        TIC277298771 & 1.1826848 & 0.02933444 & 0.05709452 & 0.04321448 & 1.6908529 & 2.3194847 & 2.005169 & 0.7058824 & 0.88505745 & 0.79546994 & 0.6414439 & 0.15820436 & 0.39982414 & 1.1770407 & 1.1798627 \\ \hline
        TIC278725797 & 4.461168 & 0.030442035 & 0.023397436 & 0.026919736 & 0.6002376 & 1.6159364 & 1.1080871 & 0.23809524 & 0.22222222 & 0.23015873 & 0.04924597 & 0.19485943 & 0.1220527 & 2.1837177 & 3.3224428 \\ \hline
        TIC278731274 & 0.4976184 & 0.09049208 & 0.057371795 & 0.07393193 & 3.6014256 & 3.231874 & 3.4166498 & 0.33333334 & 0.33333334 & 0.33333334 & 0.70606333 & 1.5074104 & 1.1067369 & 0.4989719 & 0.49829516 \\ \hline
        TIC278825715 & 6.5202184 & 0.006672227 & 0.022857143 & 0.014764685 & 0.6002381 & 2.05551 & 1.3278741 & 0.6666667 & 0.75 & 0.7083333 & 0.02743491 & 0.22437423 & 0.12590457 & 6.437734 & 6.4789762 \\ \hline
        TIC300651846 & ~ & ~ & 0.0013912629 & 0.0013912629 & ~ & 0.68575764 & 0.68575764 & 0.2972973 & 0.11111111 & 0.2042042 & 0.09154184 & 0.03961221 & 0.06557702 & 0.34409007 & 0.34409007 \\ \hline
        TIC306574570 & 10.131888 & 0.0 & ~ & 0.0 & 0.0 & ~ & 0.0 & 0.04255319 & 0.121212125 & 0.081882656 & 0.036966123 & 0.027079102 & 0.032022614 & ~ & 10.131888 \\ \hline
        TIC31381302 & 0.16519958 & 0.008610792 & 0.016335372 & 0.012473082 & 0.548576 & 1.8981893 & 1.2233826 & 0.14285715 & 0.0882353 & 0.11554622 & 0.028145997 & 0.03307552 & 0.030610759 & 0.16527405 & 0.16523682 \\ \hline
        TIC33866201 & 0.257622 & 0.003966505 & 0.0061963773 & 0.0050814413 & 0.3159346 & 0.6857016 & 0.5008181 & 0.05 & 0.14814815 & 0.09907407 & 0.028264308 & 0.018113807 & 0.023189057 & 0.25743547 & 0.25752872 \\ \hline
        TIC350145729 & 4.845551 & 0.051260266 & 0.00873515 & 0.029997708 & 1.0195233 & 1.251761 & 1.1356422 & 0.5555556 & 0.24 & 0.39777777 & 0.06432342 & 0.05313181 & 0.058727615 & 2.6613474 & 3.7534492 \\ \hline
        TIC38698751 & 0.60303545 & 0.0 & 0.0016349888 & 8.174944E-4 & 0.0 & 0.1472417 & 0.07362085 & 0.04 & 0.12195122 & 0.08097561 & 0.04721536 & 0.06989151 & 0.058553435 & 0.6020775 & 0.60255647 \\ \hline
        TIC391946225 & ~ & ~ & 0.0031116297 & 0.0031116297 & ~ & 0.2791199 & 0.2791199 & 0.12962963 & 0.06818182 & 0.09890573 & 0.07003666 & 0.01388001 & 0.041958336 & 5.5347557 & 5.5347557 \\ \hline
        TIC55497266 & 0.32437664 & 0.0472879 & 0.08010397 & 0.06369594 & 3.0004148 & 5.272958 & 4.1366863 & 0.7818182 & 0.7297297 & 0.75577396 & 0.7216701 & 0.9945846 & 0.85812736 & 0.3241618 & 0.32426924 \\ \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

==> tables/tess_survey_info.tex <==
\begin{table}[h!]\label{tess-survey-info}
  \begin{center}
    \caption{TESS survey years (1-6), observed hemispheres, observed sectors and their respective Start and Stop dates}
    \label{tab:tess-survey-info}
    \begin{tabular}{c|c|c|c|c} % <-- Alignments: 1st column left, 2nd middle and 3rd right, with vertical lines in between
      \textbf{Year} & \textbf{ecliptic hemisphere} & \textbf{sectors} & \textbf{Start date}& \textbf{Stop date}\\
      \hline
      1 & Southern & 1-13 & 25.07.2018 & 18.07.2019\\
      2 & Northern & 14-26 & 18.07.2019 & 04.07.2020\\
      3 & Southern & 27-39 & 04.07.2020 & 24.06.2021\\
      4 & Northern & 40-55 & 24.06.2021 & 01.09.2022\\
      5 & Northern+Southern & 56-69 & 01.09.2022 & 20.09.2023\\
      6 & Southern+Northern & 70-83 & 20.09.2023 & 01.10.2024\\
    \end{tabular}
  \end{center}
\end{table}

==> tables/tic_dist_g_gbp_grp.tex <==
\begin{table}[!ht]
    \centering
    \caption{Table with the final sample's TIC ID, the integrated Gaia blue and red photometer mean magnitudes (\(G_{BP}\) and \(G_{RP}\)), the absolute Gaia G-band magnitude (\(MG\)) and the distance in parsecs (\(Distance [pc]\)).}
    \label{tab:dist-mag}
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        TIC ID & G_{BP} [mag] & G_{RP} [mag] & MG [mag] & Distance [pc] \\ \hline
        TIC391946225 & 16.783 & 13.855 & 10.352 & 89.522 \\ \hline
        TIC33866201 & 16.958 & 13.895 & 11.548 & 53.444 \\ \hline
        TIC300651846 & 16.445 & 13.574 & 9.613 & 109.996 \\ \hline
        TIC38698751 & 17.318 & 13.641 & 13.248 & 22.785 \\ \hline
        TIC260352702 & 16.576 & 13.596 & 11.633 & 44.222 \\ \hline
        TIC141422340 & 14.824 & 12.656 & 8.514 & 126.651 \\ \hline
        TIC167812509 & 16.837 & 13.163 & 13.219 & 18.519 \\ \hline
        TIC31381302 & 16.712 & 12.666 & 13.824 & 11.421 \\ \hline
        TIC278825715 & 15.047 & 12.261 & 9.542 & 61.394 \\ \hline
        TIC150301109 & 15.055 & 12.582 & 10.264 & 49.061 \\ \hline
        TIC167894019 & 16.933 & 12.632 & 12.9 & 17.456 \\ \hline
        TIC306574570 & 12.694 & 9.977 & 9.405 & 22.508 \\ \hline
        TIC140758953 & 16.14 & 13.411 & 10.754 & 59.373 \\ \hline
        TIC278731274 & 14.465 & 11.92 & 8.418 & 85.46 \\ \hline
        TIC350145729 & 16.041 & 13.238 & 9.407 & 102.567 \\ \hline
        TIC55497266 & 12.286 & 10.015 & 9.128 & 24.555 \\ \hline
        TIC277298771 & 12.373 & 10.384 & 7.742 & 52.971 \\ \hline
        TIC141156752 & 16.292 & 13.497 & 10.128 & 83.189 \\ \hline
        TIC220395392 & 14.976 & 12.177 & 10.066 & 46.42 \\ \hline
        TIC177257889 & 15.162 & 12.953 & 8.933 & 103.815 \\ \hline
        TIC150359500 & 12.614 & 9.829 & 10.383 & 13.446 \\ \hline
        TIC260189734 & 15.755 & 13.055 & 9.286 & 98.927 \\ \hline
        TIC278725797 & 14.494 & 12.323 & 8.214 & 107.457 \\ \hline
        TIC220473309 & 10.325 & 8.406 & 7.204 & 26.901 \\ \hline
        TIC142052608 & 16.133 & 13.177 & 11.431 & 39.886 \\ \hline
    \end{tabular}
\end{table}

==> tables/tic_erass_dc.tex <==
\begin{table*}[!ht]
    \centering
    \caption{Table with TIC ID, eRASS duty cycle of eRASS 2 \((\nu_{x,DC,eRASS2})\), eRASS 3 \((\nu_{x,DC,eRASS3})\), the mean eRASS duty cycle \((\nu_{x,DC,mean})\) and the standard deviation (\(\nu_{x,DC,std.dev}\)) of the two eRASS surveys}
    \label{table:erass-dc}
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        TIC ID & $\nu_{x,DC,eRASS2}$ & $\nu_{x,DC,eRASS3}$ & $\nu_{x,DC,mean}$ & $\nu_{x,DC,std.dev}$ \\ \hline
        TIC140758953 & 0.222 & 0.278 & 0.25 & 0.028 \\ \hline
        TIC141156752 & 0.333 & 0.357 & 0.345 & 0.012 \\ \hline
        TIC141422340 & 0.12 & 0.059 & 0.089 & 0.031 \\ \hline
        TIC142052608 & 0.051 & 0.212 & 0.132 & 0.081 \\ \hline
        TIC150301109 & 0.071 & 0.143 & 0.107 & 0.036 \\ \hline
        TIC150359500 & 0.5 & 0.432 & 0.466 & 0.034 \\ \hline
        TIC167812509 & 0.219 & 0.31 & 0.265 & 0.046 \\ \hline
        TIC167894019 & 0.172 & 0.48 & 0.326 & 0.154 \\ \hline
        TIC177257889 & 0.064 & 0.057 & 0.06 & 0.004 \\ \hline
        TIC220395392 & 0.413 & 0.29 & 0.352 & 0.062 \\ \hline
        TIC220473309 & 0.674 & 0.438 & 0.556 & 0.118 \\ \hline
        TIC260189734 & 0.333 & 0.441 & 0.387 & 0.054 \\ \hline
        TIC260352702 & 0.045 & 0.034 & 0.04 & 0.006 \\ \hline
        TIC277298771 & 0.706 & 0.885 & 0.795 & 0.09 \\ \hline
        TIC278725797 & 0.238 & 0.222 & 0.23 & 0.008 \\ \hline
        TIC278731274 & 0.333 & 0.333 & 0.333 & 0.0 \\ \hline
        TIC278825715 & 0.667 & 0.75 & 0.708 & 0.042 \\ \hline
        TIC300651846 & 0.297 & 0.111 & 0.204 & 0.093 \\ \hline
        TIC306574570 & 0.043 & 0.121 & 0.082 & 0.039 \\ \hline
        TIC31381302 & 0.143 & 0.088 & 0.116 & 0.028 \\ \hline
        TIC33866201 & 0.05 & 0.148 & 0.099 & 0.049 \\ \hline
        TIC350145729 & 0.556 & 0.24 & 0.398 & 0.158 \\ \hline
        TIC38698751 & 0.04 & 0.122 & 0.081 & 0.041 \\ \hline
        TIC391946225 & 0.13 & 0.068 & 0.099 & 0.031 \\ \hline
        TIC55497266 & 0.782 & 0.73 & 0.756 & 0.026 \\ \hline
    \end{tabular}
\end{table*}

==> tables/tic_rot.tex <==
\begin{table*}[h!]
    \centering
    \caption{Table with the TIC ID, rotation period from eRASS 2 (\(P_{Rot,eRASS2}\)), eRASS 3 (\(P_{Rot,eRASS3}\)), the mean rotation period (\(P_{Rot,mean}\)) and the standard deviation (\(P_{Rot,std.dev}\)) of the two surveys in days.
    * Stars with the standard deviation normalized to the rotation period \(\geq20\%\). \textcolor{teal}{** (needs to be changed) Stars with \(P_{Rot}\) computed from the only TESS light curve that was taken during eRASS 2 or eRASS 3 but not both}}
    \label{tab:tic-rot}
    %\begin{adjustbox}{angle=90}
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        TIC ID & $P_{Rot,eRASS2}[days]$ & $P_{Rot,eRASS3}[days]$ & $P_{Rot,mean}[days]$ & $P_{Rot,std.dev}[days]$ \\ \hline
        TIC140758953 & 1.374 & 1.367 & 1.371 & 0.004 \\ \hline
        TIC141156752 & 1.417 & 1.889 & 1.653 & 0.236 \\ \hline
        TIC141422340 & 13.64 & 11.396 & 12.518 & 1.122 \\ \hline
        TIC142052608 & 2.984 & 2.936 & 2.96 & 0.024 \\ \hline
        TIC150301109* & 2.621 & 1.007 & 1.814 & 0.807 \\ \hline
        TIC150359500** & 1.029 & ~ & 1.029 & ~ \\ \hline
        TIC167812509 & 0.336 & 0.336 & 0.336 & 0.0 \\ \hline
        TIC167894019* & 3.912 & 1.188 & 2.55 & 1.362 \\ \hline
        TIC177257889 & 11.651 & 10.206 & 10.929 & 0.723 \\ \hline
        TIC220395392** & ~ & 5.066 & 5.066 & ~ \\ \hline
        TIC220473309 & 8.795 & 8.601 & 8.698 & 0.097 \\ \hline
        TIC260189734 & 17.288 & 15.586 & 16.437 & 0.851 \\ \hline
        TIC260352702** & ~ & 1.003 & 1.003 & ~ \\ \hline
        TIC277298771 & 1.183 & 1.177 & 1.18 & 0.003 \\ \hline
        TIC278725797* & 4.461 & 2.184 & 3.322 & 1.139 \\ \hline
        TIC278731274 & 0.498 & 0.499 & 0.498 & 0.001 \\ \hline
        TIC278825715 & 6.52 & 6.438 & 6.479 & 0.041 \\ \hline
        TIC300651846** & ~ & 0.344 & 0.344 & ~ \\ \hline
        TIC306574570** & 10.132 & ~ & 10.132 & ~ \\ \hline
        TIC31381302 & 0.165 & 0.165 & 0.165 & 0.0 \\ \hline
        TIC33866201 & 0.258 & 0.257 & 0.258 & 0.001 \\ \hline
        TIC350145729* & 4.846 & 2.661 & 3.753 & 1.093 \\ \hline
        TIC38698751 & 0.603 & 0.602 & 0.603 & 0.001 \\ \hline
        TIC391946225** & ~ & 5.535 & 5.535 & ~ \\ \hline
        TIC55497266 & 0.324 & 0.324 & 0.324 & 0.0 \\ \hline
    \end{tabular}
    %\end{adjustbox}
\end{table*}

==> tables/tic_rot_new.tex <==
\begin{table*}[h!]
    \centering
    \caption{Table with the TIC ID, rotation period from eRASS 2 (\(P_{Rot,eRASS2}\)), eRASS 3 (\(P_{Rot,eRASS3}\)), the mean rotation period (\(P_{Rot,mean}\)) and the standard deviation (\(P_{Rot,std.dev}\)) of the two surveys in days.
    \textcolor{teal}{x the highest peak in the periodogram was not atleast twice as high as the second highest peak
    ** Badly de-trended light curves.
    * `double-dipped' light curves, where the longer period was chosen as the 'true' period}.}
    \label{tab:tic-rot}
    %\begin{adjustbox}{angle=90}
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        TIC ID & $P_{Rot,eRASS2}[days]$ & $P_{Rot,eRASS3}[days]$ & $P_{Rot,std.dev}[days]$ \\ \hline
        TIC140758953 & 1.374 & 1.367 & 0.007 \\ \hline
        TIC141156752 & x & x & ~ \\ \hline
        TIC141422340 & x & x & ~ \\ \hline
        TIC142052608 & 2.984 & 2.936 & 0.048 \\ \hline
        TIC150301109 & x & x & ~ \\ \hline
        TIC150359500 & 1.029 & ~ & ~ \\ \hline
        TIC167812509 & x & 0.336 & ~ \\ \hline
        TIC167894019 & x & x & ~ \\ \hline
        TIC177257889 & ** & x** & ~ \\ \hline
        TIC220395392 & ~ & 5.066 & ~ \\ \hline
        TIC220473309 & x & 8.601 & ~ \\ \hline
        TIC260189734 & x & x & ~ \\ \hline
        TIC260352702 & ~ & 1.003 & ~ \\ \hline
        TIC277298771 & 1.183 & 1.177 & 0.006 \\ \hline
        TIC278725797 & 4.461 & x & ~ \\ \hline
        TIC278731274 & 0.498 & 0.499 & 0.001 \\ \hline
        TIC278825715 & 6.52 & 6.438 & 0.082 \\ \hline
        TIC300651846 & ~ & 0.344 & ~ \\ \hline
        TIC306574570 & x & ~ & ~ \\ \hline
        TIC31381302 & 0.165 & 0.165 & 0.0 \\ \hline
        TIC33866201 & *0.258 & *0.257 & 0.001 \\ \hline
        TIC350145729 & x & *2.661 & ~ \\ \hline
        TIC38698751 & 0.603 & 0.602 & 0.001 \\ \hline
        TIC391946225 & ~ & 5.535 & ~ \\ \hline
        TIC55497266 & 0.324 & 0.324 & 0.0 \\ \hline
    \end{tabular}
    %\end{adjustbox}
\end{table*}

==> tables/tic_rot_rqui.tex <==
\begin{table}[!ht]
    \centering
    \caption{Table with the TIC ID, rotation period from eRASS 2 (\(P_{Rot,e2}\)), eRASS 3 (\(P_{Rot,e3}\)), the mean rotation period (\(P_{Rot,mean}\)) and the standard deviation (\(P_{Rot,std.dev}\)) of the two surveys in days, quiescent rate from eRASS 2 (\(R_{qui,e2}\)), eRASS 3 (\(R_{qui,e3}\)), the mean quiescent rate (\(R_{qui,mean})\)) and the standard deviation (\(R_{qui,std.dev}\)) from the two surveys.}
    \label{table:rot-rqui}
    \begin{adjustbox}{angle=90}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
    \hline
        TIC ID & P_{Rot,e2}[days] & P_{Rot,e3}[days] & P_{Rot,mean}[days] & P_{Rot,std.dev}[days] & R_{qui,e2} & R_{qui,e3} & R_{qui,mean} &  R_{qui,std.dev} \\ \hline
        TIC140758953 & 1.374 & 1.367 & 1.371 & 0.004 & 0.004 & 0.027 & 0.016 & 0.012 \\ \hline
        TIC141156752 & 1.417 & 1.889 & 1.653 & 0.236 & 0.026 & 0.026 & 0.026 & 0.0 \\ \hline
        TIC141422340 & 13.64 & 11.396 & 12.518 & 1.122 & 0.016 & 0.006 & 0.011 & 0.005 \\ \hline
        TIC142052608 & 2.984 & 2.936 & 2.96 & 0.024 & 0.004 & 0.011 & 0.008 & 0.004 \\ \hline
        TIC150301109 & 2.621 & 1.007 & 1.814 & 0.807 & 0.029 & 0.029 & 0.029 & 0.0 \\ \hline
        TIC150359500 & 1.029 & ~ & 1.029 & ~ & 2.517 & 1.828 & 2.172 & 0.345 \\ \hline
        TIC167812509 & 0.336 & 0.336 & 0.336 & 0.0 & 0.018 & 0.005 & 0.012 & 0.007 \\ \hline
        TIC167894019 & 3.912 & 1.188 & 2.55 & 1.362 & 0.024 & 0.062 & 0.043 & 0.019 \\ \hline
        TIC177257889 & 11.651 & 10.206 & 10.929 & 0.723 & 0.006 & 0.017 & 0.011 & 0.006 \\ \hline
        TIC220395392 & ~ & 5.066 & 5.066 & ~ & 0.325 & 0.305 & 0.315 & 0.01 \\ \hline
        TIC220473309 & 8.795 & 8.601 & 8.698 & 0.097 & 3.605 & 4.603 & 4.104 & 0.499 \\ \hline
        TIC260189734 & 17.288 & 15.586 & 16.437 & 0.851 & 0.024 & 0.062 & 0.043 & 0.019 \\ \hline
        TIC260352702 & ~ & 1.003 & 1.003 & ~ & 0.042 & 0.015 & 0.028 & 0.014 \\ \hline
        TIC277298771 & 1.183 & 1.177 & 1.18 & 0.003 & 0.641 & 0.158 & 0.4 & 0.242 \\ \hline
        TIC278725797 & 4.461 & 2.184 & 3.322 & 1.139 & 0.049 & 0.195 & 0.122 & 0.073 \\ \hline
        TIC278731274 & 0.498 & 0.499 & 0.498 & 0.001 & 0.706 & 1.507 & 1.107 & 0.401 \\ \hline
        TIC278825715 & 6.52 & 6.438 & 6.479 & 0.041 & 0.027 & 0.224 & 0.126 & 0.099 \\ \hline
        TIC300651846 & ~ & 0.344 & 0.344 & ~ & 0.092 & 0.04 & 0.066 & 0.026 \\ \hline
        TIC306574570 & 10.132 & ~ & 10.132 & ~ & 0.037 & 0.027 & 0.032 & 0.005 \\ \hline
        TIC31381302 & 0.165 & 0.165 & 0.165 & 0.0 & 0.028 & 0.033 & 0.031 & 0.003 \\ \hline
        TIC33866201 & 0.258 & 0.257 & 0.258 & 0.001 & 0.028 & 0.018 & 0.023 & 0.005 \\ \hline
        TIC350145729 & 4.846 & 2.661 & 3.753 & 1.093 & 0.064 & 0.053 & 0.059 & 0.006 \\ \hline
        TIC38698751 & 0.603 & 0.602 & 0.603 & 0.001 & 0.047 & 0.07 & 0.059 & 0.012 \\ \hline
        TIC391946225 & ~ & 5.535 & 5.535 & ~ & 0.07 & 0.014 & 0.042 & 0.028 \\ \hline
        TIC55497266 & 0.324 & 0.324 & 0.324 & 0.0 & 0.722 & 0.995 & 0.858 & 0.137 \\ \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

==> tables/tic_rqui.tex <==
\begin{table*}[h!]
    \centering
    \caption{Table with the TIC ID,
    quiescent rate from eRASS 2 (\(R_{qui,eRASS2}\)), eRASS 3 (\(R_{qui,eRASS3}\)), the mean quiescent rate (\(R_{qui,mean}\)) and the standard deviation (\(R_{qui,std.dev}\)) from the two surveys in cts/sec.}
    \label{table:tic-rqui}
  %  \begin{adjustbox}{angle=90}
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        TIC ID & R\_{qui,eRASS2}[cts/sec] & R\_{qui,eRASS3}[cts/sec] & R\_{qui,mean}[cts/sec] & R\_{qui,std.dev}[cts/sec] \\ \hline
        TIC140758953 & 0.004 & 0.027 & 0.016 & 0.012 \\ \hline
        TIC141156752 & 0.026 & 0.026 & 0.026 & 0.0 \\ \hline
        TIC141422340 & 0.016 & 0.006 & 0.011 & 0.005 \\ \hline
        TIC142052608 & 0.004 & 0.011 & 0.008 & 0.004 \\ \hline
        TIC150301109 & 0.029 & 0.029 & 0.029 & 0.0 \\ \hline
        TIC150359500 & 2.517 & 1.828 & 2.172 & 0.345 \\ \hline
        TIC167812509 & 0.018 & 0.005 & 0.012 & 0.007 \\ \hline
        TIC167894019 & 0.024 & 0.062 & 0.043 & 0.019 \\ \hline
        TIC177257889 & 0.006 & 0.017 & 0.011 & 0.006 \\ \hline
        TIC220395392 & 0.325 & 0.305 & 0.315 & 0.01 \\ \hline
        TIC220473309 & 3.605 & 4.603 & 4.104 & 0.499 \\ \hline
        TIC260189734 & 0.024 & 0.062 & 0.043 & 0.019 \\ \hline
        TIC260352702 & 0.042 & 0.015 & 0.028 & 0.014 \\ \hline
        TIC277298771 & 0.641 & 0.158 & 0.4 & 0.242 \\ \hline
        TIC278725797 & 0.049 & 0.195 & 0.122 & 0.073 \\ \hline
        TIC278731274 & 0.706 & 1.507 & 1.107 & 0.401 \\ \hline
        TIC278825715 & 0.027 & 0.224 & 0.126 & 0.099 \\ \hline
        TIC300651846 & 0.092 & 0.04 & 0.066 & 0.026 \\ \hline
        TIC306574570 & 0.037 & 0.027 & 0.032 & 0.005 \\ \hline
        TIC31381302 & 0.028 & 0.033 & 0.031 & 0.003 \\ \hline
        TIC33866201 & 0.028 & 0.018 & 0.023 & 0.005 \\ \hline
        TIC350145729 & 0.064 & 0.053 & 0.059 & 0.006 \\ \hline
        TIC38698751 & 0.047 & 0.07 & 0.059 & 0.012 \\ \hline
        TIC391946225 & 0.07 & 0.014 & 0.042 & 0.028 \\ \hline
        TIC55497266 & 0.722 & 0.995 & 0.858 & 0.137 \\ \hline
    \end{tabular}
    %\end{adjustbox}
\end{table*}

==> tables/tic_sec.tex <==
\begin{table}[!ht]
    \centering
    \caption{Table with the final star sample's TIC ID, the number of TESS sectors they were observed in (max=13) (\(N_{sectors}\)), and the sectors they were observed in (S27-S39; 1= Observed in sector, 0= Not observed in sector)}
    \label{tab:tic-sec}
    \begin{adjustbox}{rotate=90}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
        TIC ID & N_{sectors} & S27 & S28 & S29 & S30 & S31 & S32 & S33 & S34 & S35 & S36 & S37 & S38 & S39 \\ \hline
        TIC391946225 & 8 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 1 & 1 & 1 & 1 & 0 & 1 \\ \hline
        TIC33866201 & 10 & 0 & 0 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC300651846 & 8 & 0 & 0 & 0 & 0 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC38698751 & 10 & 0 & 0 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC260352702 & 12 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC141422340 & 12 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC167812509 & 13 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC31381302 & 10 & 0 & 1 & 1 & 0 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC278825715 & 13 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC150301109 & 11 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 \\ \hline
        TIC167894019 & 12 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC306574570 & 12 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC140758953 & 13 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC278731274 & 13 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC350145729 & 12 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 \\ \hline
        TIC55497266 & 12 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC277298771 & 12 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC141156752 & 13 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC220395392 & 11 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 \\ \hline
        TIC177257889 & 12 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC150359500 & 11 & 0 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 \\ \hline
        TIC260189734 & 12 & 1 & 1 & 1 & 1 & 1 & 1 & 0 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC278725797 & 13 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC220473309 & 13 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 \\ \hline
        TIC142052608 & 12 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 0 \\ \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

==> tables/tic_tessfr_tessdc.tex <==
\begin{table*} %[h!]
    \centering
    \caption{\textcolor{orange}{Optical variability diagnostics derived from TESS light curves.} TIC ID, TESS flare rate from eRASS 2 ($\nu_{\rm o,f,eRASS2}$) and eRASS 3 ($\nu_{\rm o,f,eRASS3}$), the TESS duty cycle from eRASS 2 ($\nu_{\rm o,DC,eRASS2}$), eRASS 3 ($\nu_{\rm o,DC,eRASS3}$) and the mean ($\nu_{\rm o,DC,mean}$) and standard deviation ($\nu_{\rm o,DC,stdev}$) between the duty cycles measured from the two surveys.}
    \label{table:tessdc-tessfr}
    \begin{tabular}{lllllll}
    \hline
        TIC ID & $\nu_{\rm o,f,eRASS2}$ & $\nu_{\rm o,f,eRASS3}$ & $\nu_{\rm o,DC,eRASS2}$ & $\nu_{\rm o,DC,eRASS3}$ & $\nu_{\rm o,DC,mean}$ & $\nu_{\rm o,DC,stdev}$ \\ 
        & [${\rm d^{-1}}$] & [${\rm d^{-1}}$] & & & & \\
        \hline
        TIC140758953 & 0.157 & 0.167 & 0.002 & 0.003 & 0.003 & 0.001 \\ %\hline
        TIC141156752 & 0.077 & 0.208 & 0.003 & 0.004 & 0.003 & 0.001 \\ %\hline
        TIC141422340 & 0.077 & 0.042 & 0.001 & 0.001 & 0.001 & 0.0 \\ %\hline
        TIC142052608 & 0.039 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\ %\hline
        TIC150301109 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\ %\hline
        TIC150359500 & 0.905 & ~ & 0.026 & ~ & 0.026 & ~ \\ %\hline
        TIC167812509 & 0.079 & 0.076 & 0.001 & 0.001 & 0.001 & 0.0 \\ %\hline
        TIC167894019 & 0.118 & 0.267 & 0.003 & 0.004 & 0.004 & 0.001 \\ %\hline
        TIC177257889 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 \\ %\hline
        TIC220395392 & ~ & 0.077 & ~ & 0.001 & 0.001 & ~ \\ %\hline
        TIC220473309 & 0.926 & 1.283 & 0.03 & 0.032 & 0.031 & 0.001 \\ %\hline
        TIC260189734 & 0.039 & 0.043 & 0.0 & 0.002 & 0.001 & 0.001 \\ %\hline
        TIC260352702 & ~ & 0.171 & ~ & 0.001 & 0.001 & ~ \\ %\hline
        TIC277298771 & 0.669 & 0.525 & 0.013 & 0.016 & 0.014 & 0.002 \\ %\hline
        TIC278725797 & 0.079 & 0.294 & 0.004 & 0.005 & 0.005 & 0.001 \\ %\hline
        TIC278731274 & 0.472 & 0.588 & 0.013 & 0.012 & 0.013 & 0.001 \\ %\hline
        TIC278825715 & 0.079 & 0.294 & 0.001 & 0.004 & 0.002 & 0.002 \\ %\hline
        TIC300651846 & ~ & 0.155 & ~ & 0.0 & 0.0 & ~ \\ %\hline
        TIC306574570 & 0.0 & ~ & 0.0 & ~ & 0.0 & ~ \\ %\hline
        TIC31381302 & 0.154 & 0.335 & 0.003 & 0.003 & 0.003 & 0.0 \\ %\hline
        TIC33866201 & 0.039 & 0.084 & 0.001 & 0.001 & 0.001 & 0.0 \\ %\hline
        TIC350145729 & 0.195 & 0.179 & 0.01 & 0.001 & 0.006 & 0.005 \\ %\hline
        TIC38698751 & 0.0 & 0.013 & 0.0 & 0.0 & 0.0 & 0.0 \\ %\hline
        TIC391946225 & ~ & 0.08 & ~ & 0.001 & 0.001 & ~ \\ %\hline
        TIC55497266 & 1.136 & 1.2 & 0.019 & 0.019 & 0.019 & 0.0 \\ 
        \hline
    \end{tabular}
\end{table*}
